Sherman: A Write-Optimized Distributed B+Tree Index on Disaggregated Memory

Memory disaggregation architecture physically separates CPU and memory into independent components, which are connected via high-speed RDMA networks, greatly improving resource utilization of databases. However, such an architecture poses unique challenges to data indexing in databases due to limited RDMA semantics and near-zero computation power at memory-side. Existing indexes supporting disaggregated memory either suffer from low write performance, or require hardware modification. This paper presents Sherman, a write-optimized distributed B+Tree index on disaggregated memory that delivers high performance with commodity RDMA NICs. Sherman combines RDMA hardware features and RDMA-friendly software techniques to boost index write performance from three angles. First, to reduce round trips, Sherman coalesces dependent RDMA commands by leveraging in-order delivery property of RDMA. Second, to accelerate concurrent accesses, Sherman introduces a hierarchical lock that exploits on-chip memory of RDMA NICs. Finally, to mitigate write amplification, Sherman tailors the data structure layout of B+Tree with a two-level version mechanism. Our evaluation shows that, Sherman is one order of magnitude faster in terms of both throughput and 99th percentile latency on typical write-intensive workloads, compared with state-of-the-art designs.

==> secs/algorithm.tex <==
\begin{algorithm}[t]
	
	\small
	\caption{Insert(key, value)}
    \label{alg:insert}
    

	
	\If(\ {\color{cmcolor}\tcp*[h]{write elimination}}){$key \in elimination\_array$  
	}{
       wait until $key \notin elimination\_array$\;
       \Return
	}
	\Else {
		add $key$ into $elimination\_array$
    }


    $leaf\_addr \gets index\_cache.find(key)$\;

    $HOCL\_Lock(leaf\_addr)$\;

    $node \gets \rread(leaf\_addr, sizeof(node))$\;
    

    $couple\_queue \gets \{\}$\ {\color{cmcolor}\tcp{\hspace{-0.1cm}RDMA task:(buffer,addr,size)}}
    \If(\ {\color{cmcolor}\tcp*[h]{insert}}){
        $\exists\ i,\ node.item[i].k == key${\ \color{cmcolor}\tcp{update}}
        $\hspace{1cm}\lor node.item[i].k == NULL$
    }{
        $node.item[i].\{k, v\} \gets \{key, value\}$\;
        $node.item[i].front\_item\_ver++$\;
        $node.item[i].rear\_item\_ver++$\;
        $couple\_queue.push(\{node, leaf\_addr + offset(item[i])$
        $, sizeof(item[i])\})$\;
    } \Else(\ {\color{cmcolor}\tcp*[h]{split}})  {
       $sibling = new\ sizeof(node)$\;
       $sibling\_addr = remote\_alloc(sizeof(node))$\;
       sort $node$, move half of items in $node$ to $sibling$\;
       $sibling.\{level, free\} \gets \{0, 1\}$\;
       link $node$ and $sibling\_node$, update their fence keys\;
       add $(key, value)$ into $node$\;
       $node.front\_node\_ver++$\;
       $node.rear\_node\_ver++$\;

       \If{
           $leaf\_addr$ and $sibling\_addr$ are in the same SN
       }{
        $couple\_queue.push(\{sibling, sibling\_addr, sizeof(node)\})$
       } \Else{
           $\rwrite(sibling, sibling\_addr, sizeof(node))$
       }
       $couple\_queue.push(\{node, leaf\_addr, sizeof(node)\})$
    }
     
    {\color{cmcolor}\tcp{unlock and \rwrite tasks in $couple\_queue$}}
    $HOCL\_Unlock(leaf\_addr, couple\_queue)$\;

    remove $key$ from $elimination\_array$\;

    if splitting nodes, insert \{$sibling.item[0].k$, $sibling\_addr$\}
    into internal nodes recursively;
	

\end{algorithm}

\begin{algorithm}[t]
	
	\small
	\caption{HOCL\_Lock(addr)}
    \label{alg:lock}

    $idx \gets hash(addr)\ \%\ kNumOfLock $\;
    $l \gets LLT[addr.sn\_id][idx]$\;
    \If(\ {\color{cmcolor}\tcp*[h]{get locks in LLT first}}){
    $lock(l)$ fails
    }{   
        $handover \gets false$\;
        $l.wait\_queue.push(\&handover)$\;
        wait until $handover$ is head of $l.wait\_queue$ and lock $l$\;
        remove head from $l.wait\_queue$\;
        \If(\ {\color{cmcolor}\tcp*[h]{be handed over}}){$handover == ture$}{ 
            \Return;
        }
    }
   
    {\color{cmcolor}\tcp{get locks in GLT finally}}
    \While{$!\rcas(\&GTL[addr.sn\_id][idx], 0, cn\_id)$}{
        ;
    }

\end{algorithm}


\begin{algorithm}[t]
	
	\small
	\caption{HOCL\_Unlock(addr, couple\_queue)}
    \label{alg:lock}

    $idx \gets hash(addr)\ \%\ kNumOfLock $\;
    $l \gets LLT[addr.sn\_id][idx]$\;
    % $l.handover\_depth++$\;

    $handover \gets LLT[idx].wait\_queue.head()$\;
    \If{$handover\ !=\ NULL$ {\ \color{cmcolor}\tcp*[h]{the queue is not empty}}\\
    $\land (++l.handover\_depth) <= kMaxDepth$} {
        {\color{cmcolor}\tcp{hand over the lock to another thread}}
        $ *handover = true$\;
    } \Else{
     $l.handover\_depth = 0$\;
     $couple\_queue.push\{0, \&GLT[addr.sn\_id][idx],2)\}$
    }

    $unlock(l)$ and \rwrite $couple\_queue$\;

    

\end{algorithm}


\begin{algorithm}[t]
	
	\small
	\caption{Search(key)}
    \label{alg:search}

    $leaf\_addr \gets index\_cache.find(key)$\;

retry:\\
\qquad $node \gets \rread(leaf\_addr, sizeof(node))$\;
\qquad \If{
    $node.front\_node\_ver$ != $node.rear\_node\_ver$
    }{
        \qquad \textbf{goto} retry;
    }
    \qquad    \If{$\exists\ e,\ e \in node \land e.k == key$}{
        \qquad    \If{
            $e.front\_item\_ver$ != $e.rear\_item\_ver$
    }{
           \qquad \textbf{goto} retry\;
           \Return e.v;
    }
    }
    \Return NULL;    

\end{algorithm}

==> secs/discussion.tex <==
%\vspace{-0.15in}
\section{Discussion}
\label{sec:discussion}

==> secs/impl.tex <==
%\vspace{-0.17in}
\section{Implementation}
